The ACRV Picking Benchmark (APB): A Robotic Shelf Picking Benchmark to Foster Reproducible Research

Robotic challenges like the Amazon Picking Challenge (APC) or the DARPA Challenges are an established and important way to drive scientific progress. They make research comparable on a well-defined benchmark with equal test conditions for all participants. However, such challenge events occur only occasionally, are limited to a small number of contestants, and the test conditions are very difficult to replicate after the main event. We present a new physical benchmark challenge for robotic picking: the ACRV Picking Benchmark (APB). Designed to be reproducible, it consists of a set of 42 common objects, a widely available shelf, and exact guidelines for object arrangement using stencils. A well-defined evaluation protocol enables the comparison of \emph{complete} robotic systems -- including perception and manipulation -- instead of sub-systems only. Our paper also describes and reports results achieved by an open baseline system based on a Baxter robot.

==> conclusion.tex <==
This paper is motivated by our experience in the recent Amazon Picking Challenge (APC).
These challenges are effective in driving reseach but are sometimes hard to reproduce. 
We propose a benchmark, with easily available physical artifacts: a standard shelf, standard set of objects, and reproducible task setups. 
%To really drive progress we believe that it is essential to make the challenge conditions more widely available.
This benchmarking task will allow for more thorough analysis, better comparison and easier reproduction of \emph{complete} robotic picking tasks.
% The benchmark is based on commonly available shelves and objects and

A major focus of the benchmark design was maximising reproducibility: %The benchmark defines
a number of carefully chosen scenarios with precise instructions on how to place, orient, and align objects with the help of printable stencils are defined. In addition a multitude of configurations can be created by combining the various stencils with all possible objects. 
We carefully selected 42 objects which vary in weight and size, and include deformable, transparent, and closely related items (baseball and softball, red and green tooth brush, full and half full water bottle).
Our hope is that the community will expand on these setups.%\footnote{The shelf description, object dataset, setups, and stencils are all available online: \url{http://Juxi.net/dataset/apb}. We hope to extend and report the communities progress on this page as well!}

% evaluation protocol for robotic picking from shelving units that fosters reproducible and thus comparable results. 
% In contrast to existing datasets, our benchmark allows to evaluate a robotic system for the \emph{complete} task, not just sub-tasks such as object detection, grasp selection, or path planning. 

The defined benchmark scenarios vary in difficulty and challenge both the manipulation capabilities as well as the perception pipeline of the evaluated robotic system.
A baseline system using a custom-off-the-shelf robot with extensions is described. It is able to perform the easy setups proposed but fails at the difficult ones. We hope the research community will take on this challenge and propose novel solutions to complete systems that improve over the baseline results presented in this paper.

% ?!This selection makes the APB benchmark a challenge for the state of the art in robotic picking.


% for the shelf picking based on a Baxter robot (depicted picking from two shelves in Fig.~\ref{fig:vis-abstract}) and report its performance on the benchmark tasks and during the 2016 APC.

% Inspired by the Amazon Picking Challenge (APC) we introduce a new \emph{physical} benchmark and evaluation protocol for robotic picking from shelving units that fosters reproducible and thus comparable results. In contrast to existing datasets, our benchmark allows to evaluate a robotic system for the \emph{complete} task, not just sub-tasks such as object detection, grasp selection, or path planning. 

% To make the benchmark as accessible as possible to the research community, a white IKEA shelf (Fig.~\ref{fig:vis-abstract}A) is used for all picking tasks, which is easily available worldwide.%, unlike the proprietary Kiva shelf used during the APC
% Furthermore, %a white IKEA Kallax shelf is used for all picking tasks, which is easily available worldwide, unlike the proprietary Kiva shelf used during the APC.
% we carefully curated a set of 42 objects (Fig.~\ref{fig:vis-abstract}B) to ensure they are widely available and are not subject to import restrictions, in contrast to some of the objects in the existing YCB dataset or the APC.


% , and comprise transparent as well as deformable objects. Some of the objects are prone of shifting their centre of mass when manipulated, 
% We grouped them into easy, medium, and hard to perceive and the same three levels of ``manipulability''.
% The configurations themselves also vary from easy, e.g.\ single object in a bin, to hard, e.g.\ various objects with occlusions, even a configuration that requires some reasoning about the scene.
% adhere strong constraints in orientation, i.e.\ they are not allowed to be turned over. 

%
